Selective "Selective Prediction": Reducing Unnecessary Abstention in Vision-Language Reasoning

Selective prediction minimizes incorrect predictions from vision-language models (VLMs) by allowing them to abstain from answering when uncertain. However, when deploying a vision-language system with low tolerance for inaccurate predictions, selective prediction may be over-cautious and abstain too frequently, even on many correct predictions. We introduce ReCoVERR, an inference-time algorithm to reduce the over-abstention of a selective vision-language system without increasing the error rate of the system's predictions. When the VLM makes a low-confidence prediction, instead of abstaining ReCoVERR tries to find relevant clues in the image that provide additional evidence for the prediction. ReCoVERR uses an LLM to pose related questions to the VLM, collects high-confidence evidences, and if enough evidence confirms the prediction the system makes a prediction instead of abstaining. ReCoVERR enables three VLMs (BLIP2, InstructBLIP, and LLaVA-1.5) to answer up to 20% more questions on the VQAv2 and A-OKVQA tasks without decreasing system accuracy, thus improving overall system reliability. Our code is available at https://github.com/tejas1995/ReCoVERR.

==> files/recoverr_algo.tex <==
\begin{comment}
    
\begin{algorithm*}
    \small
    \caption{\recoverr Algorithm}
        \KwData{
    \\$Q_{V}$: Visual question that we are trying to answer \\
    $I$: Image \\
    Models: Vision-language model $\model{VL}$, Large language model $\model{LLM}$}
    \Parameter{$\gamma_{\texttt{VL}}$ : VL model confidence threshold \\
    $\gamma_{\texttt{guess}}$ : minimum guess confidence threshold \\
    $\delta_{\texttt{defeas}}$ : minimum relevance defeasibility delta}
    \KwResult{$\hat{a}$: Answer to $Q_V$}
    \Comment{Get image caption $C$ along with confidence $P_{VL}(C | I)$}
    $C, P_{VL}(C | I) \gets \model{VL}(I)$ \\
    \If{$P_{VL}(C | I)$ > $\gamma_{\texttt{VL}}$}{
        \Comment{If caption is reliable, guess an answer for $Q_V$ based on caption}
        \texttt{agent\_guess}, \texttt{guess\_conf}  $\gets \model{LLM}(Q_V | C)$ \\
        \texttt{guess\_conf} $\gets \model{LLM}(\texttt{agent\_guess} | Q_V, C)$ \\
        \If{$\texttt{guess\_conf} > \gamma_{\texttt{guess}}$}{
            \Return \texttt{agent\_guess}
        }
    }
    \quad\\
    \Comment{Generate a set of candidate answers $\hat{A}$ for $Q_V$ from VL model, prune duplications with LLM}
    $\hat{A} = [a_1...a_5] \gets \model{VL}(Q_V, I)$ \\
    $\hat{A} \gets \model{LLM}(\hat{A})$ \Comment{Remove duplicates in $\hat{A}$} \\
    \quad\\
    \Comment{Generate a set of reliable evidences $E_{R}$}
    $E_{R} \gets []$ \\
    \For{$i \gets 1$ to $N$}{
        $Q_{1...K} \gets \model{LLM}(C, E_{R})$ \quad \Comment{Generate a set of K candidate next-questions from LLM based on caption and evidences already collected}\\
        $A_{1...K} \gets \model{VL}(Q_{1...K+1}, I)$ \quad \Comment{Get VL answers for each question}\\
        \For{$j \gets 1$ to $K$}{
            \Comment{Each ($Q_j, A_j, P_{VL}(A_j | Q_j, I)$) triple represents a new evidence, retain only reliable ones}
            \If{$P_{VL}(A_j | Q_j, I) > \gamma_{\texttt{VL}}$}{
                $E_R \gets E_R + \Big[ \Big( Q_{j}, A_{j}, P_{VL}(A_j | Q_j, I) \Big) \Big]$ \\
            }
        }
    }
    \Comment{Identify evidences $E_{RR}$ that are reliable AND relevant}
    $E_{RR} \gets []$ \\
    \For{$e$ \texttt{ in } $E_R$}{
        \texttt{agent\_guess}  $\gets \model{LLM}(Q_V | C, e)$ \Comment{Guess answer for $Q_V$ based on caption $C$ and evidence $e$}
        \texttt{guess\_conf} $\gets \model{LLM}(\texttt{agent\_guess} | Q_V, C, e)$ \Comment{Get LLM confidence for \texttt{agent\_guess} if evidence $e$ is true} \\
        \texttt{guess\_conf\_counterevidence}  $\gets \model{LLM}(\texttt{agent\_guess} | Q_V, C, \Bar{e})$ \Comment{Get LLM confidence for \texttt{agent\_guess} if evidence $e$ is false}
        \If{\texttt{guess\_conf} - \texttt{guess\_conf\_counterevidence} > $\delta_{\texttt{defeas}}$}{
            $E_{RR} \gets E_{RR} + [e]$
        }
    }

    \eIf{\texttt{len($E_{RR}$) == 0}}{
        \Comment{If no reliable and relevant evidences are found, abstain}   
        \Return $\phi$
    }{
        \Comment{Try answering the question based on gathered evidences}
        \texttt{agent\_guess}  $\gets \model{LLM}(Q_V | C, E_{RR})$ \\
        \texttt{guess\_conf} $\gets \model{LLM}(\texttt{agent\_guess} | Q_V, C, E_{RR})$ \\
        %\texttt{guess\_conf} $\gets$ \model{VL}(\texttt{agent\_guess} | $Q_V, E_{RR}, I$)\\
        \eIf{\texttt{guess\_conf} > $\gamma_{\texttt{guess}}$}{
            \Return \texttt{agent\_guess}
        }{
            \Return $\phi$ \quad \Comment{If LLM is not sufficiently confident based on gathered evidences, abstain}
        }
    }
\end{algorithm*}
\end{comment}

\begin{comment}
    
\begin{algorithm*}
    \small
    \caption{\recoverr\ Algorithm}
        \KwData{
    \\$Q_{V}$: Visual question that we are trying to answer \\
    $I$: Image \\
    Models: Vision-language model $\model{\texttt{VLM}}$, Question generation model $\model{\texttt{QGen}}$, Verifier model $\model{\texttt{Verif}}$ (either an LLM or VLM)}
    \Parameter{$r \in [0, 1]$ : desired risk \\
    $\gamma_{\texttt{VL}}$ : VLM confidence threshold corresponding to desired risk level \\
    $\delta_{\texttt{defeas}}$ : minimum relevance defeasibility delta\\
    $N$: Number of turns of evidence collection\\
    $K$: Questions generated at each turn}
    \KwResult{$\hat{a}$: Answer to $Q_V$}
    \Comment{Get VLM prediction $\answer$, along with confidence $P_{\texttt{VLM}}( \answer| \question)$}
    $\answer, P_{\texttt{VLM}}( \answer| \question) \gets \model{\texttt{VLM}}(I, \question)$ \\
    \If{$P_{\texttt{VLM}}( \answer| \question) \geq \gamma_{\texttt{VL}}$}{
        \Return $\answer$ \Comment{If confidence is higher than the threshold corresponding to desired risk level, return answer}
    }
    \quad\\
    \Comment{Get image caption $C$ along with confidence $P_{\texttt{VLM}}(C | I)$}
    $C, P_{\texttt{VLM}}(C | I) \gets \model{\texttt{VLM}}(I)$ \\
    \If{$P_{\texttt{VLM}}(C | I) > 1-r$}{
        \Comment{If caption is reliable, guess an answer for $Q_V$ based on caption}
        \texttt{guess\_conf} $\gets \model{\texttt{LLM/VLM}}(\answer | Q_V, C)$ \\
        \If{$\texttt{guess\_conf} > 1-r$}{
            \Return \texttt{agent\_guess}
        }
    }
    \quad\\
    \Comment{Generate a set of reliable evidences $E_{R}$}
    $E_{R} \gets [\ ]$ \\
    \For{$i \gets 1$ to $N$}{
        $Q_{1...K} \gets \model{\texttt{QGen}}(C, E_{R})$ \quad \Comment{Generate a set of K candidate next-questions from LLM based on caption and evidences already collected}\\
        $A_{1...K} \gets \model{\texttt{VLM}}(Q_{1...K}, I)$ \quad \Comment{Get VL answers for each question}\\
        \For{$j \gets 1$ to $K$}{
            \Comment{Each ($Q_j, A_j, P_{\texttt{VLM}}(A_j | Q_j, I)$) triple represents an evidence, retain only reliable ones}
            \If{$P_{\texttt{VLM}}(A_j | Q_j, I) > 1-r$}{
                $E_R \gets E_R + \Big[ \Big( Q_{j}, A_{j}, P_{\texttt{VLM}}(A_j | Q_j, I) \Big) \Big]$ \\
            }
        }
    }

    \quad\\
    \Comment{Identify evidences $E_{RR}$ that are reliable AND relevant}
    $E_{RR} \gets [\ ]$ \\
    \For{$e$ \texttt{ in } $E_R$}{
        \texttt{guess\_conf\_trueevidence} $\gets \model{\texttt{Verif}}(\answer | Q_V, C, e)$ \Comment{Get LLM confidence for prediction $\answer$ if evidence $e$ is true} \\
        \texttt{guess\_conf\_falseevidence}  $\gets \model{\texttt{Verif}}(\answer | Q_V, C, \Bar{e})$ \Comment{Get LLM confidence for prediction $\answer$ if evidence $e$ is false}
        \If{\mid \texttt{guess\_conf\_trueevidence} - \texttt{guess\_conf\_falseevidence} \mid > $\delta_{\texttt{defeas}}$}{
            $E_{RR} \gets E_{RR} + [e]$
        }
    }

    \eIf{\texttt{len($E_{RR}$) == 0}}{
        \Comment{If no reliable and relevant evidences are found, abstain}   
        \Return $\phi$
    }{
        \Comment{Get confidence for $\answer$ based on gathered evidences}
        \texttt{guess\_conf} $\gets \model{\texttt{Verif}}(\answer | Q_V, C, E_{RR})$ \\
        \eIf{\texttt{guess\_conf} > $1-r$}{
            \Return $\answer$
        }{
            \Return $\phi$ \quad \Comment{If Verifier is not sufficiently confident based on gathered evidences, abstain}
        }
    }
\end{algorithm*}
\end{comment}

\begin{comment}
    
\begin{algorithm*}
    \small
    \caption{\recoverr\ Algorithm}
        \KwData{
    \\$Q_{V}$: Visual question that we are trying to answer \\
    $I$: Image \\
    Models: Vision-language model $\model{\texttt{VLM}}$, Question generation model $\model{\texttt{QGen}}$, Verifier model $\model{\texttt{Verif}}$ (either an LLM or VLM)}
    \Parameter{$r \in [0, 1]$ : desired risk \\
    $\gamma_{@r}$ : VLM confidence threshold corresponding to desired risk level \\
    $\delta_{\texttt{defeas}}$ : minimum relevance defeasibility delta\\
    $N$: Maximum number of turns of evidence collection\\
    $K$: Questions generated at each turn}
    \KwResult{$\hat{a}$: Answer to $Q_V$}
    \Comment{Get VLM prediction $\answer$, along with confidence $\pi_{\texttt{VLM}}( \answer )$}
    $\answer, \pi_{\texttt{VLM}}( \answer ) \gets \model{\texttt{VLM}}(I, \question)$ \\
    \If{$\pi_{\texttt{VLM}}(\answer) \geq \gamma_{@r}$}{
        \Return $\answer$ \Comment{If confidence is higher than the threshold corresponding to desired risk level, return answer}
    }
    \quad\\
    \Comment{Get image caption $C$ along with confidence $\pi_{\texttt{VLM}}(C)$}
    $C, \pi_{\texttt{VLM}}(C) \gets \model{\texttt{VLM}}(I)$ \\
    \If{$\pi_{\texttt{VLM}}(C) > 1-r$}{
        \Comment{If caption is reliable, guess an answer for $Q_V$ based on caption}
        \texttt{guess\_conf} $\gets \model{\texttt{Verif}}(\answer | Q_V, C)$ \\
        \If{$\texttt{guess\_conf} > 1-r$}{
            \Return \texttt{agent\_guess}
        }
    }
    \quad\\
    \Comment{Generate a set of reliable evidences $E_{R}$}
    $E_{R}, E_{RR} \gets [\ ], [\ ]$ \\
    \For{$i \gets 1$ to $N$}{
        $Q_{1...K} \gets \model{\texttt{QGen}}(C, E_{R})$ \quad \Comment{Generate a set of K candidate next-questions from $\model{QGen}$ based on caption and evidences already collected}\\
        $A_{1...K}, \pi_{\texttt{VLM}}(A_{1...K}) \gets \model{\texttt{VLM}}(Q_{1...K}, I)$ \quad \Comment{Get VLM answers for each question}\\
        \For{$j \gets 1$ to $K$}{
            \Comment{Each ($Q_j, A_j, \pi_{\texttt{VLM}}(A_j)$) triple represents an evidence, retain only reliable ones}
            $e \gets \Big( Q_{j}, A_{j}, \pi_{\texttt{VLM}}(A_j) \Big)$ \\
            \If{$\pi_{\texttt{VLM}}(A_j) > 1-r$}{
                $E_R \gets E_R + [ e ]$ \\
                \Comment{Additionally, identify if evidence is relevant}
                \texttt{conf\_trueevidence} $\gets \pi_{\texttt{Verif}}(\answer | C, e)$ 
                \Comment{Get Verifier confidence for prediction $\answer$ if evidence $e$ is true} \\
                \texttt{conf\_falseevidence}  $\gets \pi_{\texttt{Verif}}(\answer | C, \Bar{e})$ \Comment{Get Verifier confidence for prediction $\answer$ if evidence $e$ is false}
                \If{\mid \texttt{conf\_trueevidence} - \texttt{conf\_falseevidence} \mid \geq $\delta_{\texttt{defeas}}$}{
                    $E_{RR} \gets E_{RR} + [e]$
                }
            }
            
        }
        \If{\texttt{len}(E_{RR}) > 0}{
            \Comment{If you have some reliable and relevant evidences, get confidence for $\answer$ based on gathered evidences}
            \texttt{conf\_aggregatedevidences} $\gets \pi_{\texttt{Verif}}(\answer | Q_V, C, E_{RR})$ \\
            \If{\texttt{conf\_aggregatedevidences} > $1-r$}{
                \Return $\answer$
            }
        }
    }
    \\
    \\
    \Comment{Unable to find enough evidences to make the Verifier sufficiently confident, so abstain}
    \Return $\varnothing$
\end{algorithm*}
\end{comment}
\begin{comment}
    
\begin{algorithm*}
    \small
    \caption{\recoverr\ Algorithm}
        \KwData{
    \\$Q_{V}$: Visual question that we are trying to answer \\
    $I$: Image \\
    Models: Vision-language model $\model{\texttt{VLM}}$, Question generation model $\model{\texttt{QGen}}$, QA re-phraser model $\model{\texttt{QA}\rightarrow\texttt{S}}$, NLI model $\model{\texttt{NLI}}$($h, p$)}
    \Parameter{$r \in [0, 1]$ : desired risk \\
    $\gamma_{@r}$ : VLM confidence threshold corresponding to desired risk level \\
    $\delta_{\texttt{defeas}}$ : minimum relevance defeasibility delta\\
    $\prob{NLImin}$: Minimum entailment confidence to answer \\
    $N$: Maximum number of turns of evidence collection\\
    $K$: Questions generated at each turn}
    %\KwResult{$\hat{a}$: Answer to $Q_V$}
    \Comment{Get VLM prediction $\answer$, along with confidence $\pi_{\texttt{VLM}}( \answer )$}
    $\answer, \pi_{\texttt{VLM}}( \answer ) \gets \model{\texttt{VLM}}(I, \question)$ \\
    \If{$\pi_{\texttt{VLM}}(\answer) \geq \gamma_{@r}$}{
        \Return $\answer$ \Comment{If confidence is higher than the threshold corresponding to desired risk level, return answer}
    }
    $S_a \gets \model{\texttt{QA}\rightarrow\texttt{S}}(Q_V, a)$ \Comment{Rephrase answer to target question into a hypothesis statement} 
    \quad\\
    \Comment{Get image caption $C$ along with confidence $\pi_{\texttt{VLM}}(C)$}
    $C, \pi_{\texttt{VLM}}(C) \gets \model{\texttt{VLM}}(I)$ \\
    \If{$\pi_{\texttt{VLM}}(C) > 1-r$}{
        \Comment{If caption is reliable, guess an answer for $Q_V$ based on caption}
        $\prob{NLI}(S_a | C) \gets \model{\texttt{NLI}}(h=S_a | p=C)$ \\
        \If{$\prob{NLI}(S_a | C)  \geq \prob{NLImin}$}{
            \Return $a$
        }
    }
    \quad\\
    \Comment{Try to recover reliable and relevant evidences $E_{RR}$ that verify the answer}
    $E_{R}, E_{RR} \gets [\ ], [\ ]$ \\
    \For{$i \gets 1$ to $N$}{
        $Q_{1...K} \gets \model{\texttt{QGen}}(C, E_{R})$ \quad \Comment{Generate a set of K candidate next-questions from $\model{QGen}$ based on caption and evidences already collected}\\
        $A_{1...K}, \pi_{\texttt{VLM}}(A_{1...K}) \gets \model{\texttt{VLM}}(Q_{1...K}, I)$ \quad \Comment{Get VLM answers for each question}\\
        \For{$j \gets 1$ to $K$}{
            $S_j \gets \model{\texttt{QA}\rightarrow\texttt{S}} (Q_j, A_j)$ \Comment{Re-phrase QA evidence into a premise sentence}\\
        
            \Comment{Each ($Q_j, A_j, \pi_{\texttt{VLM}}(A_j), S_j$) 4-tuple represents an evidence, retain only reliable ones}
            $e \gets \Big( Q_{j}, A_{j}, \pi_{\texttt{VLM}}(A_j), S_j \Big)$ \\
            \If{$\pi_{\texttt{VLM}}(A_j) > 1-r$}{
                $E_R \gets E_R + [ e ]$ \\
                \Comment{Additionally, identify if evidence is relevant}
                $\prob{NLI}(S_a | C, S_j) \gets \model{\texttt{NLI}}(h=S_a | p=\{C, S_j\})$ 
                \Comment{Get entailment confidence for prediction $\answer$ if evidence $e$ is true} \\
                $\prob{NLI}(S_a | C, \Bar{S_j}) \gets \model{\texttt{NLI}}(h=S_a | p=\{C, \Bar{S_j}\})$ 
                \Comment{Get entailment confidence for prediction $\answer$ if evidence $e$ is false} \\
                \If{$\mid \prob{NLI}(S_a | C, S_j) - \prob{NLI}(S_a | C, \Bar{S_j}) \mid \geq \delta_{\texttt{defeas}}$}{
                    $E_{RR} \gets E_{RR} + [e]$
                }
            }
            
        }
        \If{\texttt{len}(E_{RR}) > 0}{
            \Comment{If you have some reliable and relevant evidences, get confidence for $\answer$ based on gathered evidences}
            $\prob{NLI}(S_a | \texttt{aggregated\_evidences}) \gets \model{\texttt{NLI}}(h=S_a | p=\{C, E_{RR}\})$ \\
            \If{$\prob{NLI}(S_a | \texttt{aggregated\_evidences}) > \prob{NLImin}$}{
                \Return $\answer$
            }
        }
    }
    \Comment{Unable to find enough evidences to make the Verifier sufficiently confident, so abstain}
    \Return $\varnothing$
\end{algorithm*}
\end{comment}

\begin{comment}
    
\begin{algorithm*}
    \small
    \caption{\recoverr\ Algorithm}
        \KwData{
    \\$Q_{V}$: Visual question that we are trying to answer \\
    $I$: Image \\
    Models: Vision-language model $\model{\texttt{VLM}}$, Question generation model $\model{\texttt{QGen}}$, QA re-phraser model $\model{\texttt{QA}\rightarrow\texttt{S}}$, NLI model $\model{\texttt{NLI}}$($h, p$)}
    \Parameter{$r \in [0, 1]$ : desired risk \\
    $\gamma_{@r}$ : VLM confidence threshold corresponding to desired risk level \\
    $\delta_{\texttt{defeas}}$ : minimum relevance defeasibility delta\\
    $\prob{NLImin}$: Minimum entailment confidence to answer \\
    $N$: Maximum number of turns of evidence collection\\
    $K$: Questions generated at each turn}
    %\KwResult{$\hat{a}$: Answer to $Q_V$}
    \Comment{Get VLM prediction $\answer$, along with confidence $\pi_{\texttt{VLM}}( \answer )$}
    $\answer, \pi_{\texttt{VLM}}( \answer ) \gets \model{\texttt{VLM}}(I, \question)$ \\
    \If{$\pi_{\texttt{VLM}}(\answer) \geq \gamma_{@r}$}{
        \Return $\answer$ \Comment{If confidence is higher than the threshold corresponding to desired risk level, return answer}
    }
    $S_a \gets \model{\texttt{QA}\rightarrow\texttt{S}}(Q_V, a)$ \Comment{Rephrase answer to target question into a hypothesis statement} 
    \quad\\

    \Comment{Instead of abstaining, try to ReCoVERR relevant and reliable evidences}
    $C, \pi_{\texttt{VLM}}(C) \gets \model{\texttt{VLM}}(I)$ \quad \Comment{Get image caption $C$ along with confidence $\pi_{\texttt{VLM}}(C)$} 
    $O \gets \model{\texttt{ObjDet}}(I)$ \quad \Comment{Get objects $O$ from object detector}
    $E_{R}, E_{RR} \gets [ C, O ], [C, O ]$ \\
    \For{$i \gets 1$ to $N$}{
        $Q_{1...K} \gets \model{\texttt{QGen}}(E_{R})$ \quad \Comment{Generate a set of K candidate next-questions from $\model{QGen}$ based on caption and evidences already collected}\\
        $A_{1...K}, \pi_{\texttt{VLM}}(A_{1...K}) \gets \model{\texttt{VLM}}(Q_{1...K}, I)$ \quad \Comment{Get VLM answers for each question}\\
        \For{$j \gets 1$ to $K$}{
            $S_j \gets \model{\texttt{QA}\rightarrow\texttt{S}} (Q_j, A_j)$ \Comment{Re-phrase QA evidence into a premise sentence}\\
            \Comment{Compute relevance $rel_j$ of evidence}
            $\prob{NLI}(S_a | S_j) \gets \model{\texttt{NLI}}(h=S_a | p=S_j)$ 
            \Comment{Get hypothesis's entailment conf if evidence is true} \\
            $\prob{NLI}(S_a | \Bar{S_j}) \gets \model{\texttt{NLI}}(h=S_a | p=\Bar{S_j})$ \Comment{Get hypothesis's entailment conf if evidence is false} \\
            $rel_j \gets \mid \prob{NLI}(S_a | S_j) - \prob{NLI}(S_a | \Bar{S_j}) \mid $ \\
            \Comment{Each ($Q_j, A_j, \pi_{\texttt{VLM}}(A_j), S_j, rel_j$) 5-tuple represents an evidence $e_j$}
            $e_j \gets \Big( Q_{j}, A_{j}, \prob{VLM}(A_j), S_j, rel_j \Big)$ \\
            \If{$\pi_{\texttt{VLM}}(A_j) > 1-r$}{
                $E_R \gets E_R + [ e_j ]$ \Comment{Update set of reliable evidences}\\
                \If{$rel_j \geq \delta_{\texttt{defeas}}$}{
                    $E_{RR} \gets E_{RR} + [e_j]$ \Comment{Update set of reliable and relevant evidences}
                }
            }
            
        }
        
        \Comment{If you have some reliable and relevant evidences, get confidence for $\answer$ based on gathered evidences}
        %$\prob{NLI}(S_a | \texttt{aggregated\_evidences}) \gets \model{\texttt{NLI}}(h=S_a | p=\{C, E_{RR}\})$ \\
        $M \gets \texttt{len}(E_{RR})$ \\
        $\prob{NLI}(S_a | \texttt{aggregated\_evidences}) \gets \frac{\sum_{j=1}^{M} rel_j \cdot \{ \prob{VLM}(A_j) \prob{NLI}(S_a | S_j) +  (1-\prob{VLM}(A_h))\prob{NLI}(S_a | \Bar{S_j})\} }{\sum_{j=1}^{M} rel_j}$ \\
            \If{$\prob{NLI}(S_a | \texttt{aggregated\_evidences}) > \prob{NLImin}$}{
                \Return $\answer$
            }
    }
    \Comment{Unable to find enough evidences to make the Verifier sufficiently confident, so abstain}
    \Return $\varnothing$
\end{algorithm*}
\end{comment}


\begin{algorithm}[t]
    \small
    \caption{\recoverr\ (Simplified)}
        \KwData{
    \\$Q_{V}$: Visual question that we are trying to answer \\
    $I$: Image \\
    \textbf{Models:} \\
    $\model{\texttt{VLM}}$: Vision-language model \\
    $\model{\texttt{ObjDet}}, \model{\texttt{RegCap}}$: Object detection and region captioning models \\
    $\model{\texttt{QGen}}$: Question generation model \\
    $\model{\texttt{QA}\rightarrow\texttt{S}}$: QA re-phraser model \\
    $\model{\texttt{NLI}}$($h, p$): NLI model \\
    \textbf{Hyper-parameters:} \\
    $r \in [0, 1]$ : desired risk \\
    $\gamma_{@r}$ : VLM confidence threshold corresponding to desired risk level \\
    $\delta_{\texttt{defeas}}$ : minimum relevance defeasibility delta\\
    $\prob{NLImin}$: Minimum entailment confidence to answer \\
    $N$: Maximum number of turns of evidence collection\\
    $K$: Questions generated at each turn \\ \quad}
    %\KwResult{$\hat{a}$: Answer to $Q_V$}
    \Comment{Get VLM prediction $\answer$, along with confidence $\pi_{\texttt{VLM}}( \answer )$}
    $\answer, \pi_{\texttt{VLM}}( \answer ) \gets \model{\texttt{VLM}}(I, \question)$ \\
    \If{$\pi_{\texttt{VLM}}(\answer) \geq \gamma_{@r}$}{
        \Return $\answer$  
    }

    \Comment{If not confident enough, try to verify answer by \recoverr-ing evidences}
    
    $C_I \gets \model{\texttt{VLM}}(I)$ \quad \Comment{Get image caption $C$} 
    $O \gets \model{\texttt{ObjDet}}(I)$ \quad \Comment{Get objects $O$ from object detector}
    $C_{Reg} \gets \model{\texttt{RegCap}}(I)$ \quad \Comment{Get region captions}
    $E_{R}, E_{RR} \gets [ C_I, O, C_{Reg} ], [C, O, C_{Reg} ]$ \\
    \For{$i \gets 1$ to $N$}{
        %Collect $K$ new visual evidences $e_{1...K}$, based on information already collected in $E_R$ \\
        $e_{1...K} \gets K $ new evidences from $\model{\texttt{QGen}}$'s questions and $\model{\texttt{VLM}}$'s answers \\ 
        \For{$j \gets 1$ to $K$}{
            \If{$e_j$ is reliable}{
                $E_R \gets E_R + [e_j]$
            }
            \If{$e_j$ is reliable and relevant}{
                $E_{RR} \gets E_{RR} + [e_j]$
            }
        }
        \Comment{Use $\model{NLI}$ to get entailment confidence of answer hypothesis, given evidences $E_{RR}$ as premise}
        $\prob{NLI} \gets \model{\texttt{NLI}}$(entailment | hypothesis=$\answer$, premise=$E_{RR}$) \\
        \If{$\prob{NLI} \geq \prob{NLImin}$}{
            \Return $\answer$
        }
    }
    \Comment{Unable to find enough evidences to make the NLI model sufficiently confident, so abstain}
    \Return $\varnothing$
\end{algorithm}





